Using Interventions to Improve Out-of-Distribution Generalization of Text-Matching Recommendation Systems

Given a user's input text, text-matching recommender systems output relevant items by comparing the input text to available items' description, such as product-to-product recommendation on e-commerce platforms. As users' interests and item inventory are expected to change, it is important for a text-matching system to generalize to data shifts, a task known as out-of-distribution (OOD) generalization. However, we find that the popular approach of fine-tuning a large, base language model on paired item relevance data (e.g., user clicks) can be counter-productive for OOD generalization. For a product recommendation task, fine-tuning obtains worse accuracy than the base model when recommending items in a new category or for a future time period. To explain this generalization failure, we consider an intervention-based importance metric, which shows that a fine-tuned model captures spurious correlations and fails to learn the causal features that determine the relevance between any two text inputs. Moreover, standard methods for causal regularization do not apply in this setting, because unlike in images, there exist no universally spurious features in a text-matching task (the same token may be spurious or causal depending on the text it is being matched to). For OOD generalization on text inputs, therefore, we highlight a different goal: avoiding high importance scores for certain features. We do so using an intervention-based regularizer that constraints the causal effect of any token on the model's relevance score to be similar to the base model. Results on Amazon product and 3 question recommendation datasets show that our proposed regularizer improves generalization for both in-distribution and OOD evaluation, especially in difficult scenarios when the base model is not accurate.

==> files/DONOTUSE_experiments.tex <==
\section{Experiments}

Colored+Rotated MNIST (CRMNIST)
\begin{itemize}
    \item Model: MLP (DomainBed)
    \item Number of steps: 5001
    \item Batch Size: 64
\end{itemize}

\subsection{Sweeps.}
\label{sec:app:sweeps}
The sweeps are given in Table \ref{tab:app:sweeps}.

\begin{table}[ht]
    \scriptsize
    \centering
    \begin{tabular}{cp{5cm}}
         {\bf Method} & {\bf Sweeps}\\ \toprule
         
         MLP & learning rate: [1e-2, 1e-3, 1e-4, 1e-5] \newline weight decay: 0 \\  \midrule
         IRM & learning rate: [1e-2, 1e-3, 1e-4, 1e-5] \newline $\lambda$: [0.01, 0.1, 1, 10, 100] \newline iterations annealing: [10, 100, 1000]\\ \midrule
         MMD & learning rate: [1e-2, 1e-3, 1e-4, 1e-5] \newline $\lambda$: [0.1, 1, 10, 100] \newline $\gamma$: [0.01, 0.0001, 0.000001\\ \midrule
         Our MMD (using correct causal constraints) & learning rate: [1e-2, 1e-3, 1e-4, 1e-5] \newline $\lambda$: [0.1, 1, 10, 100] \newline $\gamma$: [0.01, 0.0001, 0.000001\\ \midrule
         
    \end{tabular}
    \caption{We perform sweeps over each of the methods for three seeds. The maximum total sweep size is twenty models per seed. For each seed, the best model (based on ID or OOD validation) is selected.}
    \label{tab:app:sweeps}
\end{table}


==> files/cut_theory.tex <==
\subsection{Comparison with Output Regularization}

Theorem 1 : Every solution of \oldreg is also a solution of \newreg

Proof : 
\input{files/tables/circles}

Consider this alternate form of \newreg where instead of difference of squares of norms, we take difference of norms. Also we use $f$ as abbrevation for $f_{\theta}$ and $f_0$ as abbrevation for $f_{\theta_0}$ 
\begin{align*}
 &||f(X)-f(X')|-|f_0(X)-f_0(X')||\\
\leq &|f(X)-f(X')-f_0(X)+f_0(X')|\\
= &|(f(X)-f_0(X))-(f(X')-f_0(X'))|\\
\leq & |f(X)-f_0(X)|+|f(X')-f_0(X')|\\
\leq & 2 \underset{X,X'}{\textrm{max}}|f(X)-f_0(X)|\\
\end{align*}

This gives us that \newreg is $\leq$ twice of \oldreg. Hence all solutions of \oldreg also also solution of \newreg
\parik{Doesn't seem to be the case. \oldreg only claims $f(X) = f_0(X)$ and doesn't guarantee $f(X') = f_0(X')$, which is assumed above}

\parik{We can claim that \oldreg being 0 keeps embeddings of ALL and ONLY training points to be the same. Non-training sentence embeddings can be anything, but it doesn't matter much given that if all training sentences are equal, no learning will happen }

Theorem? 2 : There exists solution of \newreg which are not solutions of \oldreg

Proof : We consider a simple bag of words model, where each sentence's representation is given by the average of its token embeddings, normalised to unit norm.

For warmup we consider that we just have 3 tokens in 2 dimensional space. These tokens are namely $x_1,x_2,x_3$ and are unit norm and have equal angle between them i.e. $x_i^\intercal x_j$ is 0.5 $\forall i,j i\neq j$. Consider that there are 2 sentences in our corpus i.e. $\{x_1,x_2\}$ and $\{x_2,x_3\}$. We start with the initial token embeddings of $\{\bar{x}_1,\bar{x}_2,\bar{x}_3\}$

Consider the \newreg regularisation for sentence 1 i.e. $X = \{x_1,x_2\}$. We have 2 possible masks (masking $x_1$ or masking $x_2$) which yields 2 equations : 

\begin{align*}
    f(\{x_1,x_2\})^\intercal f(\{x_1\}) &= f(\{\bar{x}_1,\bar{x}_2\})^\intercal f(\{\bar{x}_1\}) \\
    f(\{x_1,x_2\})^\intercal f(\{x_2\}) &= f(\{\bar{x}_1,\bar{x}_2\})^\intercal f(\{\bar{x}_2\}) \\
\end{align*}

The first equation can be written as 
$$
\frac{(x_1+x_2)^\intercal x_2}{\sqrt{(x_1+x_2)^\intercal (x_1+x_2)}} = \frac{(\bar{x}_1+\bar{x}_2)^\intercal \bar{x}_2}{\sqrt{(\bar{x}_1+\bar{x}_2)^\intercal (\bar{x}_1+\bar{x}_2)}}
$$
And similarly the second equation can be symmetrically opened up.
One of the possible solution of the above two equations by inspection is 
\begin{align*}
    x_1^\intercal x_1 &= \bar{x}_1^\intercal \bar{x}_1\\
    x_1^\intercal x_2 &= \bar{x}_1^\intercal \bar{x}_2\\
    x_2^\intercal x_2 &= \bar{x}_2^\intercal \bar{x}_2\\
\end{align*}

Similarly, for second sentence  $X = \{x_2,x_3\}$, a possible solution for 

\begin{align*}
    x_2^\intercal x_2 &= \bar{x}_2^\intercal \bar{x}_2\\
    x_2^\intercal x_3 &= \bar{x}_2^\intercal \bar{x}_3\\
    x_3^\intercal x_3 &= \bar{x}_3^\intercal \bar{x}_3\\
\end{align*}

Assume that $\bar{x}_1 = (\frac{\sqrt{3}}{2},\frac{1}{2})$,
$\bar{x}_2 = (\frac{-\sqrt{3}}{2},\frac{1}{2})$,
$\bar{x}_3 = (0,-1)$

then 
${x}_1 = (\frac{\sqrt{3}}{2},\frac{1}{2})$,
${x}_2 = (\frac{-\sqrt{3}}{2},\frac{1}{2})$,
${x}_3 = (\frac{\sqrt{3}}{2},\frac{1}{2})$

is a valid solution for \newreg as it satisfies all the conditions. But it isn't a solution for \oldreg as $\hat{({x}_2+{x}_3)} \neq \hat{(\bar{x}_2+\bar{x}_3)}$

Generalising this for $N$ dimension we get any solution that satisfies $ x_i^\intercal x_j = \bar{x}_i^\intercal \bar{x}_j $, where $i,j$ co-occur in a sentence($i$ can be $= j$) is a valid solution for \newreg, while it might not be the case for \oldreg 

Hence we have shown that all solutions for \oldreg are valid for \newreg and that there are solutions for \newreg which are not valid for \oldreg. Hence \newreg's solution space is strictly? bigger than \oldreg's solution space. 


==> files/tables/new_tables.tex <==


\begin{table*}[tbh]
%\setlength\tabcolsep{3pt} % default value: 6pt
\small
\centering
% \begin{tabularx}{\textwidth}{lll|ll}
% \begin{tabularx}{\textwidth}{@{} *{5}{L} @{}}
\begin{tabular}{lllll}
\hline
\multirow{2}{*}{Fine-tuning Method} & \multicolumn{2}{c}{Temporal Shift} & \multicolumn{2}{c}{Categorical Shift} \\
& \textbf{Amazon131K (IID)} & \textbf{Amazon1.3M (OOD)} & \textbf{AmazonCatRemoved (IID)} & \textbf{AmazonCatOOD (OOD)} \\
% & \textbf{IID (131K/\{5 Cat\})} & \textbf{OOD (5 cats)} & \textbf{IID(131K)} & \textbf{OOD (1.3M)} \\
\hline

\base & 22.50 & 25.71 & 20.01 & 30.61  \\\cline{1-5}  
\stdfine & \textbf{39.71 $\pm$ 0.14} & 26.02 $\pm$ 0.08 & \textbf{38.74 $\pm$ 0.08} & 28.31 $\pm$ 0.17 \\\cline{1-5} 
\maskreg & 39.56 $\pm$ 0.01 & 26.65 $\pm$ 0.02 & 37.92 $\pm$ 0.11 & 29.09 $\pm$ 0.06 \\\cline{1-5}
\simcse & 39.47 $\pm$ 0.11 & 26.05 $\pm$ 0.02 & 38.05 $\pm$ 0.56 & 28.52 $\pm$ 0.10 \\\cline{1-5}    
\oldreg & 38.03 $\pm$ 0.53 & \textbf{27.60 $\pm$ 0.03} & 37.66 $\pm$ 0.11 & \textbf{31.21 $\pm$ 0.03} \\\cline{1-5}
\oldinter & - & - & 37.73 & 30.95 \\\cline{1-5}
\newreg & \textbf{39.72 $\pm$ 0.10} & 27.08 $\pm$ 0.01  & \textbf{38.77 $\pm$ 0.02} & 29.53 $\pm$ 0.04\\\cline{1-5}


\hline
% \end{tabularx}
\end{tabular}
\caption{P@1 for Temporal and Categorical Shifts on \textit{Amazon Titles}. }%.See Sec~\ref{sec:amz-data}}
\label{tab:reco}
\vspace*{-5pt}
\end{table*}



\begin{table*}[tbh]
%\setlength\tabcolsep{3pt} % default value: 6pt
\small
\centering
% \begin{tabularx}{\textwidth}{lll|ll}
% \begin{tabularx}{\textwidth}{@{} *{5}{L} @{}}
\begin{tabular}{lll}
\hline

{Fine-tuning Method} & \textbf{AmazonCatRemoved (IID)} & \textbf{Amazon131K (IID+OOD)}\\
\hline

\base & 20.01 & 21.31   \\ 
\hline
\stdfine & 38.63 & 37.06 \\ 
\hline
\maskreg & 37.92 & 36.63 \\
\hline
\simcse  & 38.41 & 36.94 \\    
\hline
\oldreg & 37.75 & 36.70 \\
\hline
\oldinter & 37.73 & 36.65 \\
\hline
\newreg  & 38.81 & 37.43\\


\hline
% \end{tabularx}
\end{tabular}
\caption{P@1 for Temporal and Categorical Shifts on \textit{Amazon Titles}. }%.See Sec~\ref{sec:amz-data}}
\label{tab:reco}
\vspace*{-5pt}
\end{table*}


==> files/tables/quora_ablations.tex <==
% \begin{table*}
% \centering
% \begin{tabular}{lllll}
% \hline
% \textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{Quora} & \textbf{AskUbuntu} & \textbf{Superuser}\\
% \hline

% \multirow{6}{*}{NLI-DistilBERT-Base} & No Finetune & \multicolumn{3}{c}{79.57} \\\cline{2-5}  
% & Std Finetune & 87.48 $\pm$ 0.19& 78.62 $\pm$ 0.62& 78.35 $\pm$ 0.18 \\\cline{2-5} 
% & \oldreg& 88.84 $\pm$ 0.27& 79.69 $\pm$ 0.02& 79.74 $\pm$ 0.24 \\\cline{2-5}
% & \maskreg & 88.85 $\pm$ 0.35& 77.57 $\pm$ 0.69& 77.50 $\pm$ 0.06 \\\cline{2-5}
% & SimCSE & 88.18 $\pm$ 0.22& 78.43 $\pm$ 0.55& 78.16 $\pm$ 0.27 \\\cline{2-5}
% % & \newreg (0.15) & 57.19 $\pm$ 0.57 & 19.70 $\pm$ 1.33 & 28.67 $\pm$ 0.26  \\\cline{2-5}    
% & \newreg & 87.96 $\pm$ 0.34& 78.59 $\pm$ 0.42& 78.90 $\pm$ 0.08  \\\cline{1-5}    

% \multirow{6}{*}{MSMARCO-DistilBERT-v4} & No Finetune & \multicolumn{3}{c}{83.41}  \\\cline{2-5}  
% & Std Finetune & 88.43 $\pm$ 0.27& 80.41 $\pm$ 0.42& 80.16 $\pm$ 0.31 \\\cline{2-5} 
% & \oldreg & 91.30 $\pm$ 0.20& 83.00 $\pm$ 0.15& 83.08 $\pm$ 0.20 \\\cline{2-5}
% & \maskreg& 89.35 $\pm$ 0.06& 77.79 $\pm$ 0.49& 78.20 $\pm$ 0.23 \\\cline{2-5}
% & SimCSE& 88.60 $\pm$ 0.16& 79.97 $\pm$ 0.44& 79.71 $\pm$ 0.45\\\cline{2-5}
% % & \newreg (0.15) & 56.63 $\pm$ 0.65 & 20.09 $\pm$ 1.46 & 33.06 $\pm$ 1.65 \\\cline{2-5}    
% & \newreg & 88.91 $\pm$ 0.29& 81.23 $\pm$ 0.27& 81.42 $\pm$ 0.25\\\cline{1-5}    


% \hline
% \end{tabular}
% \caption{\label{quora}
% Evaluated on Quora}
% \end{table*}


% \begin{table*}
% \small
% \centering
% \begin{tabular}{lllll}
% \hline
% \textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{Quora} & \textbf{AskUbuntu} & \textbf{Superuser}\\
% \hline

% \multirow{6}{*}{NLI-DistilBERT-Base} & \base & 14.00 & \textbf{14.00} & \textbf{14.00} \\\cline{2-5}  
% & \stdfine & 33.22 $\pm$ 0.82& 12.74 $\pm$ 0.43& 12.82 $\pm$ 0.49 \\\cline{2-5} 
% & \maskreg& \textbf{35.02 $\pm$ 0.85} & 12.44 $\pm$ 0.48& 13.13 $\pm$ 0.17 \\\cline{2-5}
% & \simcse & 32.52 $\pm$ 0.29& 12.87 $\pm$ 0.36& 13.41 $\pm$ 0.20 \\\cline{2-5}
% % & \newreg (0.15) & 33.94 $\pm$ 1.47 & 13.62 $\pm$ 0.25 & 14.35 $\pm$ 0.28  \\\cline{2-5}    
% & \oldreg& 33.41 $\pm$ 0.70& \textbf{14.09 $\pm$ 0.18} & \textbf{14.44 $\pm$ 0.28} \\\cline{2-5}
% & \newreg & 32.93 $\pm$ 0.49& 13.57 $\pm$ 0.32& 14.67 $\pm$ 0.18 \\\cline{1-5}    

% \multirow{6}{*}{MSMARCO-DistilBERT-v4} & \base &18.39 &  \textbf{18.39} & \textbf{18.39}  \\\cline{2-5}  
% & \stdfine & 34.15 $\pm$ 0.30& 14.05 $\pm$ 0.19& 14.35 $\pm$ 0.20 \\\cline{2-5} 
% & \maskreg& 36.49 $\pm$ 0.70& 12.63 $\pm$ 0.36& 13.65 $\pm$ 0.20 \\\cline{2-5}
% & \simcse& 34.85 $\pm$ 1.32& 14.98 $\pm$ 0.08& 14.70 $\pm$ 0.05\\\cline{2-5}
% % & \newreg (0.15) & 38.41 $\pm$ 1.09 & 15.61 $\pm$ 0.22 & 15.94 $\pm$ 0.15 \\\cline{2-5}    
% & \oldreg & \textbf{38.50 $\pm$ 0.29}& 17.16 $\pm$ 0.13& 17.64 $\pm$ 0.25 \\\cline{2-5}
% & \newreg & 35.26 $\pm$ 1.09& 16.11 $\pm$ 0.36& 16.39 $\pm$ 0.31\\\cline{1-5}    


% \hline
% \end{tabular}
% \caption{\label{exp:quora_ablation}
% AUC (0.05) numbers on Quora using two different base models NLI-DistilBERT-Base and MSMARCO-DistilBERT-Base. Different columns denote different training datasets. \base is the best model for large domain shifts}
% \end{table*}



\begin{table}
\small
\centering
\begin{tabular}{llll}
\hline
\textbf{Base Model} & \textbf{Method} & \textbf{AskUbuntu} & \textbf{Superuser}\\
\hline

\multirow{6}{*}{NLI} & \base& \textbf{14.00} & \textbf{14.00} \\\cline{2-4}  
& \stdfine & 12.74 $\pm$ 0.43& 12.82 $\pm$ 0.49 \\\cline{2-4} 
& \maskreg & 12.44 $\pm$ 0.48& 13.13 $\pm$ 0.17 \\\cline{2-4}
& \simcse& 12.87 $\pm$ 0.36& 13.41 $\pm$ 0.20 \\\cline{2-4}
% & \newreg (0.15) & 33.94 $\pm$ 1.47 & 13.62 $\pm$ 0.25 & 14.35 $\pm$ 0.28  \\\cline{2-5}    
& \oldreg& \textbf{14.09 $\pm$ 0.18} & \textbf{14.44 $\pm$ 0.28} \\\cline{2-4}
& \newreg& 13.57 $\pm$ 0.32& 14.67 $\pm$ 0.18 \\\cline{1-4}    

\multirow{6}{*}{MSMARCO} & \base &  \textbf{18.39} & \textbf{18.39}  \\\cline{2-4}  
& \stdfine& 14.05 $\pm$ 0.19& 14.35 $\pm$ 0.20 \\\cline{2-4} 
& \maskreg& 12.63 $\pm$ 0.36& 13.65 $\pm$ 0.20 \\\cline{2-4}
& \simcse& 14.98 $\pm$ 0.08 & 14.70 $\pm$ 0.05\\\cline{2-4}
% & \newreg (0.15) & 38.41 $\pm$ 1.09 & 15.61 $\pm$ 0.22 & 15.94 $\pm$ 0.15 \\\cline{2-5}    
& \oldreg & 17.16 $\pm$ 0.13& 17.64 $\pm$ 0.25 \\\cline{2-4}
& \newreg & 16.11 $\pm$ 0.36& 16.39 $\pm$ 0.31\\\cline{1-4}    


\hline
\end{tabular}
\caption{\label{exp:quora_ablation}
AUC (0.05) on \textit{Quora} using two base models, NLI-DistilBERT-Base and MSMARCO-DistilBERT-Base. Columns denote different training datasets. \base is the best model given the extreme domain shift.}
\end{table}



==> files/tables/reco_inter.tex <==
\begin{figure}[tb]
\centering
\begin{tikzpicture}%[scale=0.50]
\begin{groupplot}[group style={group size= 1 by 1},width=0.42\textwidth,height=0.25\textwidth]
\nextgroupplot[
% ybar=1.0pt, 
tick label style={font=\small},
% symbolic x coords={Climate,Electricity,JantaHack,M5},
% xtick={Climate,Electricity,JantaHack,M5},
% xtick={Tail,,,,,,Head},
% xtick={0,2,4,6,8},
% xtick={0,1,2,3,4,5,6,7,8,9},
xtick={0,3,6,9,12,15,18,21,24,27},
% ytick={-0.5,-0.25,0,0.25,0.5},
ytick={-0.5,0},
% xtick={0,1,2,3,4,5,6,7,8,9},
xtick pos=left,
ytick pos=left,
% bar shift=20.0pt,
% x=0.9cm,
% style={xshift=0pt,yshift=0pt,anchor=north,font=\footnotesize},
% xticklabels={,Tail,,,,Head,,},
scaled y ticks = false,
legend pos = north west, 
% ymin=0,
% tickwidth=0pt,
ymajorgrids=true,
ylabel = {\footnotesize P@1 Difference},
xlabel = {\footnotesize Percentage of 1.3M Items (OOD) Added},
legend style={at={(1.0,0.0)},anchor=south east,legend columns=2,font=\scriptsize },
%title=MCAR,
%legend to name=fred,
% bar width=5pt
]
% \addplot[gray,mark=*] coordinates {(0, 0) (3, 0) (6, 0) (9, 0) (12, 0) (15, 0) (18, 0) (21, 0) (24, 0) (27, 0)  };
\addplot[brown!40!black,mark=square*] coordinates {(0, -0.139) (3, -0.144) (6, -0.076) (9, -0.025) (12, -0.033) (15, 0.020) (18, 0.050) (21, 0.079) (24, 0.073) (27, 0.100)};
\addplot[cyan!40!black,mark=triangle*] coordinates {(0, -0.342) (3, -0.283) (6, -0.233) (9, -0.173) (12, -0.164) (15, -0.092) (18, -0.103) (21, -0.100) (24, -0.050) (27, -0.062)};
%[yellow!10!black, fill=yellow!80!black]    
%[blue, fill=blue!40!white]
%[gray, fill=black!40!white]
\addplot[red,mark=star] coordinates {(0, -0.699) (3, -0.534) (6, -0.387) (9, -0.217) (12, -0.096) (15, 0.054) (18, 0.111) (21, 0.228) (24, 0.250) (27, 0.348)  };
\addplot[blue,mark=diamond*] coordinates { (0, -0.019) (3, 0.017) (6, 0.055) (9, 0.098) (12, 0.128) (15, 0.154) (18, 0.198) (21, 0.266) (24, 0.254) (27, 0.264) };

% \legend{\stdfine,\oldreg,\maskreg,\simcse,\newreg};
\legend{\maskreg,\simcse,\oldreg,\newreg};
\coordinate (c1) at (rel axis cs:0,1);

\end{groupplot}

\end{tikzpicture}
% \vspace*{-20pt}
\caption{\label{exp:reco_inter} To simulate temporal evolution,  we start with \textit{Amazon131K} and add 39K new items %(and their corresponding queries) 
from \textit{Amazon1.3M} dataset at each tick.  \newreg is the only method that is consistently better than \stdfine on P@1.}% and hence on right end we have 482K items.  % \oldreg surpasses \newreg as the  start doing comparable to Finetuned model as we get more new labels with \oldreg finally surpassing \newreg. These numbers are averaged over ten runs}
\label{fig:barplots}
% \vspace*{-15pt}
\end{figure}

%errors

% cat_regeval_more (0, -0.699) (1, -0.534) (2, -0.387) (3, -0.217) (4, -0.096) (5, 0.054) (6, 0.111) (7, 0.228) (8, 0.250) (9, 0.348) [0.         0.06460693 0.0753847  0.06321909 0.09743752 0.09073631
%  0.07690929 0.08191735 0.07287428 0.02315495]
% cat_diffreg_more (0, -0.019) (1, 0.017) (2, 0.055) (3, 0.098) (4, 0.128) (5, 0.154) (6, 0.198) (7, 0.266) (8, 0.254) (9, 0.264) [0.         0.06470775 0.0735269  0.06277493 0.10030634 0.08326871
%  0.08786833 0.06488224 0.04713237 0.05454744]
% cat_simcse_more (0, -0.342) (1, -0.283) (2, -0.233) (3, -0.173) (4, -0.164) (5, -0.092) (6, -0.103) (7, -0.100) (8, -0.050) (9, -0.062) [0.         0.04707955 0.06710141 0.07997606 0.09640473 0.06152609
%  0.03470672 0.09179218 0.054525   0.05029202]
% cat_masked_more (0, -0.139) (1, -0.144) (2, -0.076) (3, -0.025) (4, -0.033) (5, 0.020) (6, 0.050) (7, 0.079) (8, 0.073) (9, 0.100) [0.         0.04046904 0.06865299 0.04256234 0.08263901 0.07397221
%  0.074267   0.07037051 0.08173458 0.06557367]

==> files/tables/sprint.tex <==
\begin{table*}
\centering
\begin{tabular}{llllll}
\hline
\textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{Quora} & \textbf{AskUbuntu} & \textbf{Superuser} & \textbf{Sprint}\\
\hline

\multirow{6}{*}{NLI-DistilBERT-Base} & No Finetune & 14.00 & 31.80 & 48.50 & 74.30 \\\cline{2-6}  
& Std Finetune & 12.48 $\pm$ 0.60 & 45.24 $\pm$ 2.38 & 63.01 $\pm$ 0.95 & 97.22 $\pm$ 0.32 \\\cline{2-6} 
& \oldreg & 11.27 $\pm$ 0.72 & 22.82 $\pm$ 0.42 & 30.84 $\pm$ 1.37 & 84.07 $\pm$ 5.17 \\\cline{2-6}
& \maskreg & 12.32 $\pm$ 0.35 & 24.83 $\pm$ 1.87 & 43.45 $\pm$ 3.10 & 95.92 $\pm$ 2.32 \\\cline{2-6}
& SimCSE & 12.71 $\pm$ 0.46 & 35.54 $\pm$ 8.61 & 59.57 $\pm$ 3.57 & 97.48 $\pm$ 0.29 \\\cline{2-6}
% & \newreg Aug (1.2x) & 12.81 & 35.71 & 53.37 & 97.86 \\\cline{2-6}
& \newreg (0.15) & 12.85 $\pm$ 0.52 & 35.90 $\pm$ 3.19 & 53.87 $\pm$ 3.80 & 98.19 $\pm$ 0.50 \\\cline{2-6}    
& \newreg (0.50) & 12.44 $\pm$ 0.61 & 34.69 $\pm$ 2.49 & 48.60 $\pm$ 4.47 & 98.15 $\pm$ 0.49 \\\cline{1-6}    

% \multirow{4}{*}{NLI-Roberta-Base-v2} & No Finetune & 3.94 & 16.48 & 25.40 & 57.04 \\\cline{2-6}  
% & Std Finetune & 8.98 & 38.32 & 35.84 & 94.44\\\cline{2-6} 
% & \oldreg & 4.49 & 12.25 & 16.47 & 75.69 \\\cline{2-6}
% & \newreg & 8.33 & 22.20 & 29.47 & 96.77 \\\cline{1-6}    

\multirow{5}{*}{MSMARCO-DistilBERT-v4} & No Finetune & 18.39 & 54.01 & 80.73 & 97.45 \\\cline{2-6}  
& Std Finetune & 13.73 $\pm$ 0.55 & 44.40 $\pm$ 3.40 & 60.17 $\pm$ 2.87 & 98.02 $\pm$ 0.09\\\cline{2-6} 
& \oldreg & 16.30 $\pm$ 0.35 & 51.04 $\pm$ 0.91 & 76.93 $\pm$ 1.57 & 97.88 $\pm$ 0.28 \\\cline{2-6}
& \maskreg & 12.99 $\pm$ 0.58 & 30.43 $\pm$ 2.88 & 50.14 $\pm$ 4.36 & 98.07 $\pm$ 0.34 \\\cline{2-6}
& SimCSE & 13.69 $\pm$ 0.26 & 43.92 $\pm$ 6.43 & 62.05 $\pm$ 3.64 & 98.18 $\pm$ 0.13 \\\cline{2-6}
% & \newreg Aug(1.2x) & 14.72 & 47.58 & 67.39 & 98.95 \\\cline{2-6}
& \newreg (0.15) & 14.53 $\pm$ 0.62 & 44.19 $\pm$ 0.51 & 67.09 $\pm$ 3.60 & 98.71 $\pm$ 0.14 \\\cline{2-6}    
& \newreg (0.50) & 14.64 $\pm$ 0.83 & 48.27 $\pm$ 1.08 & 71.93 $\pm$ 0.85 & 98.77 $\pm$ 0.09 \\\cline{1-6}    

\hline
\end{tabular}
\caption{\label{sprint}
Trained on Sprint}
\end{table*}



==> files/tables/sprint10.tex <==

\begin{table*}
\centering
\begin{tabular}{llllll}
\hline
\textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{Quora} & \textbf{AskUbuntu} & \textbf{Superuser} & \textbf{Sprint}\\
\hline

\multirow{6}{*}{NLI-DistilBERT-Base} & No Finetune & 14.00 & 31.80 & 48.50 & 74.30 \\\cline{2-6}  
& Std Finetune & 12.49 $\pm$ 0.45 & 39.41 $\pm$ 3.65 & 56.63 $\pm$ 2.45 & 91.86 $\pm$ 0.41 \\\cline{2-6} 
& \oldreg & 11.41 $\pm$ 0.38 & 21.53 $\pm$ 1.55 & 28.76 $\pm$ 2.30 & 75.34 $\pm$ 3.07 \\\cline{2-6}
& \maskreg & 11.43 $\pm$ 0.42 & 13.43 $\pm$ 2.23 & 26.49 $\pm$ 4.00 & 84.25 $\pm$ 0.85 \\\cline{2-6}
& SimCSE & 12.26 $\pm$ 0.21 & 32.72 $\pm$ 6.30 & 46.68 $\pm$ 7.10 & 89.60 $\pm$ 0.88\\\cline{2-6}
& \newreg (0.15) & 12.66 $\pm$ 0.73 & 30.05 $\pm$ 1.93 & 47.78 $\pm$ 3.50 & 90.25 $\pm$ 0.98\\\cline{2-6}    
% & \newreg Aug (1.2x) & 12.81 & 35.71 & 53.37 & 97.86 \\\cline{2-6}
& \newreg (0.50) & 13.41 $\pm$ 0.40 & 37.67 $\pm$ 2.34 & 52.42 $\pm$ 4.29 & 91.54 $\pm$ 0.72\\\cline{1-6}    

% \multirow{4}{*}{NLI-Roberta-Base-v2} & No Finetune & 3.94 & 16.48 & 25.40 & 57.04 \\\cline{2-6}  
% & Std Finetune & 8.98 & 38.32 & 35.84 & 94.44\\\cline{2-6} 
% & \oldreg & 4.49 & 12.25 & 16.47 & 75.69 \\\cline{2-6}
% & \newreg & 8.33 & 22.20 & 29.47 & 96.77 \\\cline{1-6}    

\multirow{5}{*}{MSMARCO-DistilBERT-v4} & No Finetune & 18.39 & 54.01 & 80.73 & 97.45 \\\cline{2-6}  
& Std Finetune & 14.69 $\pm$ 0.85 & 48.14 $\pm$ 6.28 & 59.25 $\pm$ 13.02 & 95.35 $\pm$ 0.40\\\cline{2-6} 
& \oldreg & 16.14 $\pm$ 0.23 & 51.44 $\pm$ 2.17 & 78.32 $\pm$ 0.15 & 96.66 $\pm$ 0.08\\\cline{2-6}
& \maskreg & 12.04 $\pm$ 0.71 & 9.55 $\pm$ 2.27 & 18.10 $\pm$ 3.48 & 86.21 $\pm$ 0.34 \\\cline{2-6}
& SimCSE & 15.46 $\pm$ 0.31 & 42.08 $\pm$ 4.64 & 62.24 $\pm$ 2.50 & 94.39 $\pm$ 0.08\\\cline{2-6}
% & \newreg Aug(1.2x) & 14.72 & 47.58 & 67.39 & 98.95 \\\cline{2-6}
& \newreg (0.15) & 15.35 $\pm$ 0.52 & 46.15 $\pm$ 1.97 & 68.68 $\pm$ 0.78 & 95.42 $\pm$ 0.34\\\cline{2-6}    
& \newreg (0.50) & 15.52 $\pm$ 0.55 & 52.48 $\pm$ 2.33 & 74.59 $\pm$ 0.50 & 96.64 $\pm$ 0.04\\\cline{1-6}    

\hline
\end{tabular}
\caption{\label{sprint}
Trained on 10\% Sprint}
\end{table*}


==> files/tables/spurious_quora.tex <==
\begin{table*}
\centering
\begin{tabular}{llll}
\hline
\textbf{Fine-tuning Method} & \textbf{Quora Complete} & \textbf{Biasing Removed} & \textbf{Only Biasing}\\
\hline
No Finetune & 14.00 & & \\
\hline
Std Finetune & 10.53 & 53.60 & 14.80\\
\oldreg & 18.62 & 50.22 & 11.08 \\
SimCSE & 9.62 & 54.69 & 12.76 \\
\newreg & 14.90 & 54.66 & 14.28\\ 

\hline

\end{tabular}
\caption{\label{quora}
Trained on Modified Quora (spurious features) with NLI-DistilBERT-Base}
\end{table*}


==> files/tables/sts_captions.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{llll}
\hline
\textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{News (OOD)} & \textbf{Captions(IID)}\\
\hline

\multirow{6}{*}{NLI-DistilBERT-Base} 
& \base & 71.58 & 87.33 \\\cline{2-4} 
& \stdfine & 73.4 $\pm$ 0.09& 89.51 $\pm$ 0.06 \\\cline{2-4} 
& \maskreg & 73.79 $\pm$ 0.12 & 89.16 $\pm$ 0.03\\\cline{2-4}
& \simcse & 73.4 $\pm$ 0.13 & 89.5 $\pm$ 0.04 \\\cline{2-4}
& \oldreg & 72.66 $\pm$ 0.09 & 88.77 $\pm$ 0.04 \\\cline{2-4}
& \newreg & 73.7 $\pm$ 0.08 & 89.47 $\pm$ 0.03 \\\cline{1-4}    

% \multirow{3}{*}{NLI-Roberta-Base-v2} & Std Finetune & 80.74 $\pm$ 0.08 & 92.55 $\pm$ 0.06 \\\cline{2-4} 
% & \oldreg & 80.84 $\pm$ 0.06 & 92.67 $\pm$ 0.03 \\\cline{2-4}
% & \newreg & 80.87 $\pm$ 0.21 & 92.56 $\pm$ 0.05 \\\cline{1-4}

\multirow{6}{*}{MSMARCO-DistilBERT-v4} 
& \base & 71.01 & 87.03 \\\cline{2-4} 
& \stdfine &  71.71 $\pm$ 0.05 &  91.22 $\pm$ 0.05 \\\cline{2-4} 
& \maskreg & 72.86 $\pm$ 0.10 & 91.20 $\pm$ 0.04\\\cline{2-4}
& \simcse & 72.05 $\pm$ 0.11 & 91.28 $\pm$ 0.03\\\cline{2-4}
& \oldreg &  71.53 $\pm$ 0.02 & 91.03 $\pm$ 0.04 \\\cline{2-4}
& \newreg & 72.02 $\pm$ 0.03  & 91.35 $\pm$ 0.04 \\\cline{1-4}
\hline
\end{tabular}
\caption{\label{tab:sts-captions}
Trained on STS-b Captions and Tested on STS-b News/Forums}
\end{table*}


==> files/tables/sts_news.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{llll}
\hline
\textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{News (IID)} & \textbf{Captions(OOD)}\\
\hline

\multirow{6}{*}{NLI-DistilBERT-Base} 
& \base & 72.45& 86.89 \\\cline{2-4} 
& \stdfine & 81.59 $\pm$ 0.06& 87.36 $\pm$ 0.05 \\\cline{2-4} 
& \maskreg & 81.06 $\pm$ 0.10 & 87.55 $\pm$ 0.07 \\\cline{2-4}
& \simcse & 81.48 $\pm$ 0.09 & 87.48 $\pm$ 0.06 \\\cline{2-4}
& \oldreg & 79.88 $\pm$ 0.10 & 87.08 $\pm$ 0.05 \\\cline{2-4}
& \newreg & 81.38 $\pm$ 0.10 & 87.40 $\pm$ 0.06 \\\cline{1-4}    

% \multirow{3}{*}{NLI-Roberta-Base-v2} & Std Finetune & 85.00 $\pm$ 0.14 & 91.35 $\pm$ 0.06 \\\cline{2-4} 
% & \oldreg & 84.96 $\pm$ 0.11 & 91.89 $\pm$ 0.03 \\\cline{2-4}
% & \newreg & 85.06 $\pm$ 0.06 & 91.49 $\pm$ 0.05 \\\cline{1-4}

\multirow{6}{*}{MSMARCO-DistilBERT-v4} 
& \base & 74.58 & 86.40 \\\cline{2-4} 
& \stdfine &  82.49 $\pm$ 0.02 &  87.84 $\pm$ 0.06 \\\cline{2-4} 
& \maskreg & 82.28 $\pm$ 0.06 & 88.13 $\pm$ 0.13 \\\cline{2-4}
& \simcse & 82.46 $\pm$ 0.04 & 88.08 $\pm$ 0.12 \\\cline{2-4}
& \oldreg &  81.71 $\pm$ 0.06 & 87.37 $\pm$ 0.04 \\\cline{2-4}
& \newreg & 82.52 $\pm$ 0.13  & 87.84 $\pm$ 0.16 \\\cline{1-4}
\hline
\end{tabular}
\caption{\label{tab:sts-news}
Trained on STS-b News/Forums and Tested on STS-b Captions}
\end{table*}


==> files/tables/sts_std.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lll}
\hline
\textbf{Pre-trained Model} & \textbf{Fine-tuning Method} & \textbf{Evaluation}\\
\hline

\multirow{6}{*}{NLI-DistilBERT-Base} 
& \base &   78.37 \\\cline{2-3} 
& \stdfine & 84.73 $\pm$ 0.06 \\\cline{2-3} 
& \maskreg & 84.06 $\pm$ 0.13 \\\cline{2-3}
& \simcse & 84.59 $\pm$ 0.12 \\\cline{2-3}
& \oldreg & 83.05 $\pm$ 0.05  \\\cline{2-3}
& \newreg & 84.55 $\pm$ 0.11  \\\cline{1-3}    

% \multirow{3}{*}{NLI-Roberta-Base-v2} & Std Finetune & 87.19 $\pm$ 0.13  \\\cline{2-3} 
% & \oldreg & 87.54 $\pm$ 0.08  \\\cline{2-3}
% & \newreg & 87.35 $\pm$ 0.07  \\\cline{1-3}

\multirow{6}{*}{MSMARCO-DistilBERT-v4} 
& \base &   78.24 \\\cline{2-3} 
& \stdfine &  85.06 $\pm$ 0.06  \\\cline{2-3} 
& \maskreg & 84.94 $\pm$ 0.04  \\\cline{2-3}
& \simcse & 85.07 $\pm$ 0.04 \\\cline{2-3}
& \oldreg &  84.79 $\pm$ 0.07 \\\cline{2-3}
& \newreg & 85.26 $\pm$ 0.03  \\\cline{1-3}
\hline
\end{tabular}
\caption{\label{tab:sts-std}
Train on Train of STS-b and Tested on the test set of STS-b
}
\end{table*}

